Beyond Data, Towards Sustainability: A Sydney Case Study on Urban Digital Twins

As urban areas grapple with unprecedented challenges stemming from population growth and climate change, the emergence of urban digital twins offers a promising solution. This paper presents a case study focusing on Sydney's urban digital twin, a virtual replica integrating diverse real-time and historical data, including weather, crime, emissions, and traffic. Through advanced visualization and data analysis techniques, the study explores some applications of this digital twin in urban sustainability, such as spatial ranking of suburbs and automatic identification of correlations between variables. Additionally, the research delves into predictive modeling, employing machine learning to forecast traffic crash risks using environmental data, showcasing the potential for proactive interventions. The contributions of this work lie in the comprehensive exploration of a city-scale digital twin for sustainable urban planning, offering a multifaceted approach to data-driven decision-making.

==> Experiments.tex <==
\section{Experiments} \label{sec:experiments}

In this section, we present the outcomes of our experimentation to evaluate the performance of various machine learning models for traffic risk prediction. 

The performance of each of these techniques across different machine-learning algorithms was evaluated. Machine learning was chosen over deep learning due to the limited size of the dataset. The models used in our study include Decision Tree, Naive Bayes, Logistic Regression, Gradient Boosted Tree, and Random Forest. All machine learning algorithms were set up using the Python Sci-Kit Learn library  and fine-tuned with the HyperOpt library.

For Hyperparameter tuning using HyperOpt, a search space must be defined for the parameters to be tuned. The objective function to find the optimal set of hyperparameters that yield the best performance on the was defined as the negative value of area under the curve (AUC). AUC is preferred over F1-score or accuracy for optimization as it is more robust to class distribution disparities of the imbalanced dataset\Aamir{citation?}. AUC better assesses the model’s ability to discriminate between the classes providing more reliable measurement for classification problems and hence for optimisation. For evaluating the performance of the tuned models, various measurements including execution times, accuracy, precision, recall, weighted F1-score, AUC, and error were considered. These measurements were taken for both the training and testing datasets.

\subsubsection{The Impact of Scalling}
Notably, Decision Trees and Random Forest, insensitive to scaling, showed limited benefits or even decreased performance. Logistic Regression and Gradient Boosted Tree models, though influenced by scaling, did not significantly benefit due to dataset characteristics.
In contrast, SMOTE-EN consistently improved performance across all models when coupled with scaling, particularly for Random Forest, Decision Tree, and Gradient Boosted Tree algorithms. This method effectively addressed class imbalance, generating synthetic samples and refining the training set, leading to enhanced accuracy.

These results could be caused by the inherent challenges due to the imbalanced nature of the dataset. In such cases, models tend to be biased towards the majority class, leading to lower accuracy and AUC values for the minority class. For instance, the Gradient Boosted Tree model exhibits notably high accuracy and AUC scores due to its ability to handle imbalanced data more effectively by assigning higher weights to misclassified minority class instances during fitting. Conversely, other models like Logistic Regression and Naïve Bayes may struggle to accurately classify the minority class due to their inherent assumptions and limitations when dealing with imbalanced data. As a result, the observed performance disparities among the models can be attributed to their varying sensitivities and capabilities in handling class imbalance. 


\subsubsection{Random Under sampling}
The performance of the random under sampling technique is reported in Table \ref{tab:performanceOrgData}. The accuracy scores for the classifiers are as follows: Decision Tree - 0.630, Gradient Boosted Tree - 0.921, Logistic Regression - 0.606, Naïve Bayes - 0.645, and Random Forest - 0.794. The corresponding AUC values are: 0.749 for Decision Tree, 0.804 for Gradient Boosted Tree, 0.586 for Logistic Regression, 0.625 for Naïve Bayes, and 0.867 for Random Forest. In the testing phase, the accuracy scores are as follows: Decision Tree - 0.630, Gradient Boosted Tree - 0.809, Logistic Regression - 0.607, Naïve Bayes - 0.646, and Random Forest - 0.717. The AUC values for testing are: 0.751 for Decision Tree, 0.594 for Gradient Boosted Tree, 0.587 for Logistic Regression, 0.626 for Naïve Bayes, and 0.731 for Random Forest. 

\begin{figure*}
    \centering
      \includegraphics[width=0.98\linewidth]{BarChart1.png}
    \caption{The abbreviations used for the models in the bar chart are GBTO (Gradient Boosted Tree Original), NBRUS (Naive Bayes Random Under Sampled), SDTSE (Scaled Decision Tree SMOTE-EN), SRFAD (Scaled Random Forest ADASYN), SRFS (Scaled Random Forest SMOTE), SRFST (Scaled Random Forest SMOTE-TOMEK), GBTE (Gradient Boosted Tree ENN), GBTR (Gradient Boosted Tree RENN), and DTNM (Decision Tree NearMiss). These abbreviations represent each model performance in terms of Accuracy and AUC in the bar chart.}
    \label{fig:models}
\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{cc
>{\columncolor[HTML]{00FF00}}c 
>{\columncolor[HTML]{FFFF00}}c ccc}
\textbf{}                           & \multicolumn{1}{l}{}        & \textbf{Decision Tree} & \textbf{Gradient Boosted Tree} & \textbf{Logistic Regression} & \textbf{Naïve Bayes} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.065                  & 5.719                          & 0.063                        & 0.010                & 12.020                 \\
                                    & \textbf{Accuracy}           & 0.630                  & 0.921                          & 0.606                        & 0.645                & 0.794                  \\
                                    & \textbf{Weighted F1-Score}  & 0.676                  & 0.916                          & 0.655                        & 0.688                & 0.818                  \\
                                    & \textbf{Weighted Precision} & 0.862                  & 0.919                          & 0.764                        & 0.782                & 0.902                  \\
                                    & \textbf{Weighted Recall}    & 0.630                  & 0.921                          & 0.606                        & 0.645                & 0.794                  \\
                                    & \textbf{AUC}                & 0.749                  & 0.804                          & 0.586                        & 0.625                & 0.867                  \\
                                    & \textbf{Error}              & 0.370                  & 0.079                          & 0.394                        & 0.355                & 0.206                  \\
\multirow{-8}{*}{\textbf{Training}} & \textbf{Time (s)}           & 0.001                  & 0.048                          & 0.002                        & 0.003                & 0.184                  \\
                                    & \textbf{Accuracy}           & 0.630                  & 0.809                          & 0.607                        & 0.646                & 0.717                  \\
                                    & \textbf{Weighted F1-Score}  & 0.677                  & 0.797                          & 0.658                        & 0.690                & 0.752                  \\
                                    & \textbf{Weighted Precision} & 0.866                  & 0.788                          & 0.771                        & 0.789                & 0.839                  \\
                                    & \textbf{Weighted Recall}    & 0.630                  & 0.809                          & 0.607                        & 0.646                & 0.717                  \\
                                    & \textbf{AUC}                & 0.751                  & 0.594                          & 0.587                        & 0.626                & 0.731                  \\
\multirow{-6}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.370                  & 0.191                          & 0.393                        & 0.354                & 0.283                 
\end{tabular}
\caption{\label{tab:performanceRandomlySampled} The performance of machine learning models on the randomly under sampled dataset.}
\end{table*}


The hyperparameter tuning process led to significant improvements in the performance of various models on the imbalanced dataset.While scaling did not significantly improve the results, it still contributed to achieving higher performance across various sampled datasets and models.

As illustrated in \ref{fig:models}, the Scaled Random Forrest Model on SMOTE, ADAYSN and SMOTE-TOMEK had the best performance for traffic risk classification. Enhancing the model's interpretability, feature importance, and addressing class  imbalance issues are also areas that require attention when continuous learning is incorporated. This  future work will contribute to the continuous advancement and practical implementation of machine  learning in traffic risk prediction for the Spatial Digital Twin Project.

==> Oriognal-Traffic.tex <==
\section{Analysing Traffic Risk Based on Environmental Conditions}\label{sec:Traffic_Analysis}
%Work on traffic risk analysis will be included here. Anjitha to contribute to this section.
In today’s modern world, traffic congestion and road accidents present significant challenges to transportation systems globally. Addressing these challenges aims to create safer and efficient road networks, improve public safety, and foster economic growth. Understanding the impact of environmental conditions on traffic risk, including weather and air quality factors, is crucial for developing effective traffic management strategies. In this report, we leverage the Spatial Digital Twin for NSW Project data and employ machine learning techniques to explore and predict traffic risk based on various environmental conditions. By uncovering insights and patterns, we aim to make evidence-based decisions that can be used to optimise traffic flow, enhance road safety, and minimise the negative impacts of congestion and accidents, ultimately contributing to developing safer and more efficient transportation systems.

\subsection{Data Collection and Processing}
%The predictive (ML) part of the system will be discussed here.
Provided data, including air quality, traffic volume, incidents, and weather, is considered from the Spatial digital twin database. However, due to the inconsistent and insufficient volume of the weather data, OpenWeatherMap   was used for the collecting weather data. 

The initial dataset exhibits several inconsistencies, notably the absence of specific readings from various sites or localities due to variations in data collection practices. For instance, the air quality data was only accessible for 21 suburbs. We observed similar inconsistencies with other datasets, which consequently led to a reduction in the final dataset size. This reduction stemmed from the absence of readings for various features on the same day or location, which resulted in large number of records being incomplete and hence removed during pre-processing.

Data Processing: (1) For data collected from different sites within the same suburb or at different times of the day, the average of their reading per day was taken to make continuous features consistent. This includes the concentration of various compounds in the air (CO, NO, etc). (2) For incidents, we take the count of incidents to ensure all incidents were accounted for. We then mapped the incident count to low or high risk based on the occurrence of traffic incidents (no accident depicts low risk and vice versa). We then use a label encoder to maintain the consistency of the data type. The counts can be later used to convert the problem into multiclass classification. (3) Several duplicates were observed within the traffic incident data, and they were removed if they shared the same information as the incident report number.  (4) For weather data, we extract the maximum and minimum temperature, precipitation, humidity, wind gust, and percentage of clouds. (5) For air quality, we use concentrations of CO, NO, NO2, O3, SO2, and particulate matter (pm). (6) Traffic volume data is updated at the end of each day. Hence having that information for analysis would only allow us to make predictions after the day has passed. Furthermore, traffic volume data is manually collected and lacks information on all the sites. Previously it was found that the day of the week was more suitable feature than traffic volume as traffic volume data as traffic pattern varied throughout the week. Thus, traffic volume was disregarded, and a new feature, day of the week, was added to the final dataset. (7) From the correlation, it was noted that some features were highly correlated, such as ozone, NO, NO2 from air quality, humidity and cloud cover, and minimum and maximum temperature from weather. Thus, in-order to avoid redundancy and improve interpretability, only the features with highest correlation (Figure 1) to traffic risk is used for the analysis.  To conclude, the final dataset consists of suburbId, day of the week, maximum temperature, precipitation, humidity, wind gust, pressure, wind direction, NO, SO2, CO, NEPH, and traffic risk.

\begin{figure*}[htbp!]
\centering
\includegraphics[width=0.7\textwidth,height=0.7\textwidth]{Figures/Correlation_HeatMap.png}
\caption{Correlation Heat Map using Pearson Correlation. The main correlations were observed within same data source such as between different features of air quality data and weather data. No significant correlation was observed between the features and the traffic risk. }
\label{fig:corr_heatmap}
\end{figure*}

\subsection{Implementation Details}
Following the common machine learning practice, the dataset was split into training and testing with an 80:20 stratified split. This resulted in a training set containing 15328 samples, with 12743 for low-risk (class 0) and 2585 from high-risk (class 1), and a test set containing 3832 samples, with 3208 from low-risk and 624 from high-risk samples. This clearly shows the problem of high-class imbalance. 

To overcome this issue, various under-sampling and over-sampling on the training dataset were employed to improve the efficiency of the approach. Applied techniques for under sampling include random under-sampling, NearMiss, Edited Nearest Neighbors (ENN), and Rerepeated ENN (RENN). Similarly, oversampling includes Synthetic Minority Over-sampling Technique (SMOTE), Adaptive Synthetic Sampling (ADYSN), SMOTE with Edited Nearest Neighbors (SMOTE-EN), and SMOTE combined with Tomek links (SMOTE-TOMEK). All the sampling techniques were only performed on the training set using Python’s imbalanced learn library . The sample sizes for the training set after sampling are reported in \ref{tab:training}. 

\begin{table}[]
\begin{tabular}{lcc}
\textbf{Technique}    & \textbf{Low Risk (Class 0)} & \textbf{High Risk (Class 1)} \\
Original              & 12743                       & 2585                         \\
Random Under sampling & 2585                        & 2585                         \\
NearMiss              & 2585                        & 2585                         \\
ENN                   & 8104                        & 2585                         \\
RENN                  & 6118                        & 2585                         \\
SMOTE-EN              & 10605                       & 6801                         \\
ADAYSN                & 12753                       & 12753                        \\
SMOTE                 & 12743                       & 12743                        \\
SMOTE-TOMEK           & 12527                       & 12527                       

\end{tabular}
\caption{\label{tab:training} Training sample size before and after sampling using different techniques.}
\end{table}

The performance of each of these techniques across different machine-learning algorithms were evaluated. Machine learning was chosen over deep learning due to the limited size of the dataset. The models used in our study include Decision Tree, Naive Bayes, Logistic Regression, Gradient Boosted Tree, and Random Forest. All machine learning algorithms were set up using the Python Sci-Kit Learn library  and fine-tuned with the HyperOpt library.

For Hyperparameter tuning using HyperOpt, a search space must be defined for the parameters to be tuned. The following describes the space for various parameters chosen for tuning. 1) Decision Tree: the `criterion' parameter, determining the criterion for measuring the quality of splits, chosen from options `gini' or `entropy'. The \verb|max_depth| parameter, indicating the maximum depth of the tree, is chosen from a range between 1 and 20. The \verb|min_samples_split| and \verb|min_samples_leaf| parameters dictate the minimum number of samples required for splitting internal nodes and forming leaf nodes, respectively, both selected from a range between 2 and 20. The \verb|max_features| hyperparameter specifies the maximum number of features considered for splitting a node, and it is chosen from the options `sqrt', `log2', or None. The \verb|class_weight| parameter considers options like no class weights or balanced class weights. 2) Gradient Boosted Tree model: the number of estimators (trees) to consider within a range from 100 to 1000 with increments of 50, the maximum depth of the trees within a range from 1 to 10, and the learning rate within a logarithmic scale between $10^-5$ and 1. 

The subsample parameter is defined within the range of 0.5 to 1, reflecting the fraction of samples utilized for each tree’s training. Moreover, the minimum samples required for splitting nodes and forming leaf nodes are considered within a uniform distribution between 0.01 and 0.5. Similarly, the range for \verb|min_samples_leaf| is also uniform between 0.01 and 0.5, accommodating float values. The \verb|max_features| hyperparameter is chosen from the options of ‘sqrt’, ‘log2’, or None, determining the maximum number of features considered for each tree split. 3) Logistic Regression: the regularization strength parameter ‘C’ is sampled from a logarithmic distribution between $10^-5$ and 100, representing the inverse of regularization intensity. The ‘penalty’ parameter is chosen between ‘l1’ and ‘l2’, reflecting the type of regularization utilized. The solver option ‘liblinear’ or ‘saga’ is selected, determining the optimization algorithm. The \verb|class_weight| parameter considers options of no class weights or balanced class weights, addressing imbalanced datasets. Additionally, the \verb|max_iter| parameter is sampled within a specific range, ensuring convergence during training. 4) Naïve Bayes: the ‘priors’ parameter is chosen from options including no prior probabilities, equal priors ([0.5, 0.5]) or custom priors ([0.3, 0.7]). These priors reflect prior probabilities for the classes. The \verb|var_smoothing| parameter is sampled from a logarithmic distribution between $10^-20$ and 1, representing the smoothing parameter applied to the variance of features during probability estimation. Finally, 5) Random Forest: the \verb|n_estimators| parameter, which determines the number of trees in the forest, sampled from a range between 100 and 1000 with increments of 50. The \verb|max_depth| parameter, defining the maximum depth of the trees, is chosen from a range between 80 and 150. The \verb|min_samples_split| and \verb|min_samples_leaf| parameters dictate the minimum number of samples required for splitting internal nodes and forming leaf nodes, respectively, both selected from a range between 2 and 20. The \verb|max_features| hyperparameter is chosen from the options ‘sqrt’ or ‘log2’, specifying the maximum number of features considered for splitting a node. The ‘bootstrap’ parameter, indicating whether bootstrapping is used for sample selection, is selected as either True or False. The \verb|class_weight| parameter considers options like no class weights, balanced class weights, or balanced subsample class weights. These search spaces act as a framework for the optimizer to explore various combinations of hyperparameter values and determine which configuration results in the optimal performance of the each of the machine learning models.

The objective function to find the optimal set of hyperparameters that yield the best performance on the was defined as the negative value of area under the curve (AUC). AUC is preferred over F1-score or accuracy for optimization as it is more robust to class distribution disparities of the imbalanced dataset. AUC better assesses the model’s ability to discriminate between the classes providing more reliable measurement for classification problems and hence for optimisation. For evaluating the performance of the tuned models, various measurements including execution times, accuracy, precision, recall, weighted F1-score, AUC, and error were considered. These measurements were taken for both the training and testing datasets.

\subsection{Results}
In this section, we present the outcomes of our experimentation to evaluate the performance of various machine learning models for traffic risk prediction. 

\subsubsection{Scalling}
One of our objectives was to determine whether scaling the features had a significant influence on the performance of these models. Upon conducting the experiments (please see the attached Excel sheet for results), we observed that the application of scaling techniques did not yield a substantial impact on the overall performance of the machine learning models. In fact, for some of the models, scaling appeared to lead decrease in performance. The reasons behind the observed decrease in performance can be attributed to the inherent characteristics of the models and the nature of the scaling process. Decision Trees, Naive Bayes, and Random Forest models are not inherently sensitive to feature scaling due to their non-parametric. These models rely on discrete decisions and statistical properties that are not fundamentally influenced by the scale of the features.

Logistic Regression and Gradient Boosted Tree models, on the other hand, may be influenced by the scaling of features. However, the datasets used in this study does not exhibit strong multicollinearity or wide variations in feature scales, which are situations where scaling becomes particularly beneficial. Consequently, scaling might have introduced noise or unnecessary changes in the data, leading to the observed decline in performance in some cases. Furthermore, the interaction between scaling and sampling techniques would have contributed to the observed performance drop. Techniques like SMOTE and ADYSN generate synthetic instances based on the characteristics of existing samples. When the features of these synthetic instances are scaled, they might not align optimally with the original data distribution, potentially leading to a misalignment between the generated samples and the decision boundaries of the models.

With regard to SMOTE-EN, the performance of all the machine learning models improved with scaling, particularly significant enhancements are observed for the Random Forest, Decision Tree, and Gradient Boosted Tree algorithms. The results are shown in Table 2. SMOTE-EN effectively tackled the issue of class imbalance by generating synthetic samples for the minority class while simultaneously applying an editing step to remove noisy samples, resulting in a more refined and balanced training set. Feature scaling, on the other hand, standardized the feature values, ensuring that each feature contributed uniformly during model training.



% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t] % table* for page-wide table and we can only have two options either t or p
\begin{tabular}{l|l|
>{\columncolor[HTML]{00FF00}}l llll}
\multicolumn{2}{l}{\textbf{}}                                     & \textbf{Decision Tree} & \textbf{Logistic Regression} & \textbf{Naive Bayes} & \textbf{Gradient Boosted Tree} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.245                  & 0.062                        & 0.016                & 12.686                         & 3.054                  \\
                                    & \textbf{Accuracy}           & 0.880                  & 0.639                        & 0.712                & 0.896                          & 0.923                  \\
                                    & \textbf{Weighted F1-Score}  & 0.879                  & 0.646                        & 0.715                & 0.894                          & 0.922                  \\
                                    & \textbf{Weighted Precision} & 0.879                  & 0.671                        & 0.724                & 0.898                          & 0.926                  \\
                                    & \textbf{Weighted Recall}    & 0.880                  & 0.639                        & 0.712                & 0.896                          & 0.923                  \\
                                    & \textbf{AUC}                & 0.866                  & 0.648                        & 0.708                & 0.874                          & 0.904                  \\
\multirow{-7}{*}{\textbf{Training}} & \textbf{Error}              & 0.120                  & 0.361                        & 0.288                & 0.104                          & 0.077                  \\
                                    & \textbf{Time (s)}           & 0.004                  & 0.014                        & 0.004                & 0.053                          & 0.044                  \\
                                    & \textbf{Accuracy}           & 0.677                  & 0.584                        & 0.584                & 0.659                          & 0.647                  \\
                                    & \textbf{Weighted F1-Score}  & 0.719                  & 0.638                        & 0.637                & 0.704                          & 0.693                  \\
                                    & \textbf{Weighted Precision} & 0.857                  & 0.772                        & 0.798                & 0.857                          & 0.854                  \\
                                    & \textbf{Weighted Recall}    & 0.677                  & 0.584                        & 0.584                & 0.659                          & 0.647                  \\
                                    & \textbf{AUC}                & 0.755                  & 0.588                        & 0.632                & 0.748                          & 0.739                  \\
\multirow{-7}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.323                  & 0.416                        & 0.416                & 0.341                          & 0.353                 
\end{tabular}
\caption{\label{tab:performance} The performance of machine learning models on the scaled SMOTE-EN dataset.}
\end{table*}


For the Random Forest model, the incorporation of SMOTE-EN with scaling contributed to a more balanced class distribution in the training data. This aided in constructing a diverse ensemble of decision trees, allowing the model to capture intricate patterns and deliver better accuracy. The Decision Tree algorithm also benefited from a balanced training set achieved through SMOTE-EN, leading to more effective separation of decision boundaries for classification tasks. Similarly, the Gradient Boosted Tree model exhibited substantial performance gains, as the ensemble of shallow decision trees capitalized on the balanced training set to uncover crucial data dependencies and enhance the boosting process.

\subsubsection{Original}
Table 3 shows the results of hyper parameter tuning for the original dataset, i.e., without any sampling techniques. For the Decision Tree model, parameters like \verb|class_weight| set to ‘balanced’, ‘criterion’ using ‘entropy’, \verb|max_depth| of 5, \verb|max_features| as None, \verb|min_samples_leaf| of 13, and \verb|min_samples_split| of 8 led to optimal performance. In the case of the Gradient Boosted Tree model, a learning rate of 0.4887, \verb|max_depth| of 8, \verb|max_features| as ‘sqrt’, \verb|min_samples_leaf| of 0.0103, \verb|min_samples_split| of 0.1405, \verb|n_estimators| of 600, and ‘subsample’ of 0.5686 yielded enhanced results. The Logistic Regression model showed the best performance with ‘C’ set to 0.0189, \verb|class_weight| as ‘balanced’, \verb|max_iter| of 10264, ‘penalty’ utilizing ‘l2’, and ‘solver’ employing ‘liblinear’. Naïve Bayes performed well with ‘prior’ of [0.5,0.5] and \verb|var_smoothing| of 3.6867e-07. These fine-tuned values were then used to fit and test the machine learning models for evaluation.

\begin{table*}[t]
\begin{tabular}{|p{4cm}p{13cm}|} % use small p for left align column
\hline
\textbf{Model} & \textbf{Parameters}                                                                                                                                                                                                    \\ \hline
\textbf{Decision Tree}         & \textbf{\{‘class\_weight’: ‘balanced’, ‘criterion’: ‘entropy’, ‘max\_depth’: 5, ‘max\_features’: None, ‘min\_samples\_leaf’: 13, ‘min\_samples\_split’: 8\}}                                          \\
\textbf{Gradient Boosted Tree} & \textbf{\{‘learning\_rate’: 0.4887, ‘max\_depth’: 8, ‘max\_features’: ‘sqrt’, ‘min\_samples\_leaf’: 0.010311698290487566, ‘min\_samples\_split’: 0.1405, ‘n\_estimators’: 600, ‘subsample’: 0.5686\}} \\
\textbf{Logistic Regression}   & \textbf{\{‘C’: 0.0189, ‘class\_weight’: ‘balanced’, ‘max\_iter’: 10264, ‘penalty’: ‘l2’, ‘solver’: ‘liblinear’\}}                                                                                     \\
\textbf{Naïve Bayes}           & \textbf{\{‘priors’: {[}0.5,0.5{]}, ‘var\_smoothing’: 3.6867e-07\}}                                                                                                                                    \\
\textbf{Random Forest}         & \textbf{\{‘bootstrap’: False, ‘class\_weight’: ‘balanced’, ‘max\_depth’: 121, ‘max\_features’: ‘log2’, ‘min\_samples\_leaf’: 20, ‘min\_samples\_split’: 5, ‘n\_estimators’: 450\}}                    \\ \hline
\end{tabular}
\caption{\label{tab:Hyperparameters} Tuned Hyperparameters for the machine learning models with the original dataset.}
\end{table*}


For the original dataset, the results are outlined in Table 4. The obtained accuracies for Decision Tree, Gradient Boosted Tree, Logistic Regression, Naïve Bayes, and Random Forest are 0.630, 0.921, 0.606, 0.645, and 0.794, respectively. Additionally, the corresponding area under the curve (AUC) values are 0.749, 0.804, 0.586, 0.625, and 0.867. During testing, the accuracy scores are 0.630, 0.809, 0.607, 0.646, and 0.717, while the AUC values are 0.751, 0.594, 0.587, 0.626, and 0.731 for the same models.

These results can be caused by the inherent challenges due to the imbalanced nature of the dataset. In such cases, models tend to be biased towards the majority class, leading to lower accuracy and AUC values for the minority class. For instance, the Gradient Boosted Tree model exhibits notably high accuracy and AUC scores due to its ability to handle imbalanced data more effectively by assigning higher weights to misclassified minority class instances during fitting. Conversely, other models like Logistic Regression and Naïve Bayes may struggle to accurately classify the minority class due to their inherent assumptions and limitations when dealing with imbalanced data. As a result, the observed performance disparities among the models can be attributed to their varying sensitivities and capabilities in handling class imbalance. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\begin{tabular}{cc
>{\columncolor[HTML]{00FF00}}c 
>{\columncolor[HTML]{FFFF00}}c ccc}
\textbf{}                           & \multicolumn{1}{l}{}        & \textbf{Decision Tree} & \textbf{Gradient Boosted Tree} & \textbf{Logistic Regression} & \textbf{Naïve Bayes} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.065                  & 5.719                          & 0.063                        & 0.010                & 12.020                 \\
                                    & \textbf{Accuracy}           & 0.630                  & 0.921                          & 0.606                        & 0.645                & 0.794                  \\
                                    & \textbf{Weighted F1-Score}  & 0.676                  & 0.916                          & 0.655                        & 0.688                & 0.818                  \\
                                    & \textbf{Weighted Precision} & 0.862                  & 0.919                          & 0.764                        & 0.782                & 0.902                  \\
                                    & \textbf{Weighted Recall}    & 0.630                  & 0.921                          & 0.606                        & 0.645                & 0.794                  \\
                                    & \textbf{AUC}                & 0.749                  & 0.804                          & 0.586                        & 0.625                & 0.867                  \\
\multirow{-7}{*}{\textbf{Training}} & \textbf{Error}              & 0.370                  & 0.079                          & 0.394                        & 0.355                & 0.206                  \\
                                    & \textbf{Time (s)}           & 0.001                  & 0.048                          & 0.002                        & 0.003                & 0.184                  \\
                                    & \textbf{Accuracy}           & 0.630                  & 0.809                          & 0.607                        & 0.646                & 0.717                  \\
                                    & \textbf{Weighted F1-Score}  & 0.677                  & 0.797                          & 0.658                        & 0.690                & 0.752                  \\
                                    & \textbf{Weighted Precision} & 0.866                  & 0.788                          & 0.771                        & 0.789                & 0.839                  \\
                                    & \textbf{Weighted Recall}    & 0.630                  & 0.809                          & 0.607                        & 0.646                & 0.717                  \\
                                    & \textbf{AUC}                & 0.751                  & 0.594                          & 0.587                        & 0.626                & 0.731                  \\
\multirow{-7}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.370                  & 0.191                          & 0.393                        & 0.354                & 0.283                 
\end{tabular}
\caption{\label{tab:performanceOrgData} The performance of machine learning models on the original dataset.}
\end{table*}

Furthermore, the AUC for Gradient Boosted Tree and Random Forest drops by 20.9\% and 13.6\% for testing, while other models displayed less than 0.25\%. The reduced performance could be attributed to several underlying factors, such as complexity of the models, and overfitting. Both Gradient Boosted Tree and Random Forests are ensemble methods that combine multiple decision trees to make predictions. If the individual decision trees within the ensemble become overly complex, they could start capturing noise and outliers present in the training data. This overfitting phenomenon would lead to reduced generalization ability and, consequently, lower performance on the testing dataset.

\subsubsection{Random Under sampling}
Table \ref{tab:Tuned_Hyperparameters} shows the result of hyper parameter tuning for randomly under sampled dataset. The optimal performance of the Decision Tree was observed with parameters \verb|class_weight| set to ‘balanced’, ‘criterion’ utilizing ‘entropy’, \verb|max_depth| of 5, \verb|min_samples_leaf| of 3, and \verb|min_samples_split| of 19. Similarly, the Gradient Boosted Tree model’s performance was elevated with an optimal \verb|learning_rate| of 0.0926, \verb|max_depth| set to 2, \verb|min_samples_leaf| of 0.17560, \verb|min_samples_split| of 0.3059, \verb|n_estimators| of 800, and ‘subsample’ of 0.8788. The Logistic Regression model demonstrated optimal outcome with the parameters ‘C’ to 0.0203, adopting ‘penalty’ as ‘l1’, and utilizing the ‘saga’ ‘solver’. Naïve Bayes exhibited optimal results with ‘prior’ of [0.5,0.5] and \verb|var_smoothing| of $2.767e-06$. The Random Forest model’s performance was optimized through parameters such as ‘bootstrap’ set to false, \verb|class_weight| using \verb|balanced_subsample|, \verb|max_depth| of 150, \verb|min_samples_leaf| of 7, \verb|min_samples_split| of 11, and \verb|n_estimators| of 350.

\begin{table*}[t]
\begin{tabular}{|p{4cm}p{13cm}|} % use small p for left align column
\textbf{Model}        & \textbf{Parameters}                                                                                                                                                                  \\
Decision Tree         & \{‘class\_weight’: ‘balanced’, ‘criterion’: ‘entropy’, ‘max\_depth’: 5, ‘max\_features’: None, ‘min\_samples\_leaf’: 3, ‘min\_samples\_split’: 19\}                                  \\
Gradient Boosted Tree & \{‘learning\_rate’: 0.0926, ‘max\_depth’: 2, ‘max\_features’: None, ‘min\_samples\_leaf’: 0.17560, ‘min\_samples\_split’: 0.3059, ‘n\_estimators’: 800, ‘subsample’: 0.8788\}        \\
Logistic Regression   & \{‘C’: 0.0203, ‘class\_weight’: None, ‘max\_iter’: 10031, ‘penalty’: ‘l1’, ‘solver’: ‘saga’\}                                                                                        \\
Naïve Bayes           & \{‘priors’: {[}0.5, 0.5{]}, ‘var\_smoothing’: 2.767e-06\}                                                                                                                            \\
Random Forest         & \{‘bootstrap’: false, ‘class\_weight’: ‘balanced\_subsample’, ‘max\_depth’: 150, ‘max\_features’: ‘log2’, ‘min\_samples\_leaf’: 7, ‘min\_samples\_split’: 11, ‘n\_estimators’: 350\}
\end{tabular}
\caption{\label{tab:Tuned_Hyperparameters} Tuned Hyperparameters for the machine learning models with randomly under sampled dataset}
\end{table*}

The performance of the random under sampling technique is reported in Table \ref{tab:performanceOrgData}. The accuracy scores for the classifiers are as follows: Decision Tree - 0.630, Gradient Boosted Tree - 0.921, Logistic Regression - 0.606, Naïve Bayes - 0.645, and Random Forest - 0.794. The corresponding AUC values are: 0.749 for Decision Tree, 0.804 for Gradient Boosted Tree, 0.586 for Logistic Regression, 0.625 for Naïve Bayes, and 0.867 for Random Forest. In the testing phase, the accuracy scores are as follows: Decision Tree - 0.630, Gradient Boosted Tree - 0.809, Logistic Regression - 0.607, Naïve Bayes - 0.646, and Random Forest - 0.717. The AUC values for testing are: 0.751 for Decision Tree, 0.594 for Gradient Boosted Tree, 0.587 for Logistic Regression, 0.626 for Naïve Bayes, and 0.731 for Random Forest. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{cc
>{\columncolor[HTML]{00FF00}}c 
>{\columncolor[HTML]{FFFF00}}c ccc}
\textbf{}                           & \multicolumn{1}{l}{}        & \textbf{Decision Tree} & \textbf{Gradient Boosted Tree} & \textbf{Logistic Regression} & \textbf{Naïve Bayes} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.065                  & 5.719                          & 0.063                        & 0.010                & 12.020                 \\
                                    & \textbf{Accuracy}           & 0.630                  & 0.921                          & 0.606                        & 0.645                & 0.794                  \\
                                    & \textbf{Weighted F1-Score}  & 0.676                  & 0.916                          & 0.655                        & 0.688                & 0.818                  \\
                                    & \textbf{Weighted Precision} & 0.862                  & 0.919                          & 0.764                        & 0.782                & 0.902                  \\
                                    & \textbf{Weighted Recall}    & 0.630                  & 0.921                          & 0.606                        & 0.645                & 0.794                  \\
                                    & \textbf{AUC}                & 0.749                  & 0.804                          & 0.586                        & 0.625                & 0.867                  \\
                                    & \textbf{Error}              & 0.370                  & 0.079                          & 0.394                        & 0.355                & 0.206                  \\
\multirow{-8}{*}{\textbf{Training}} & \textbf{Time (s)}           & 0.001                  & 0.048                          & 0.002                        & 0.003                & 0.184                  \\
                                    & \textbf{Accuracy}           & 0.630                  & 0.809                          & 0.607                        & 0.646                & 0.717                  \\
                                    & \textbf{Weighted F1-Score}  & 0.677                  & 0.797                          & 0.658                        & 0.690                & 0.752                  \\
                                    & \textbf{Weighted Precision} & 0.866                  & 0.788                          & 0.771                        & 0.789                & 0.839                  \\
                                    & \textbf{Weighted Recall}    & 0.630                  & 0.809                          & 0.607                        & 0.646                & 0.717                  \\
                                    & \textbf{AUC}                & 0.751                  & 0.594                          & 0.587                        & 0.626                & 0.731                  \\
\multirow{-6}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.370                  & 0.191                          & 0.393                        & 0.354                & 0.283                 
\end{tabular}
\caption{\label{tab:performanceRandomlySampled} The performance of machine learning models on the randomly under sampled dataset.}
\end{table*}


From table \ref{tab:performanceOrgData} and \ref{tab:performanceRandomlySampled}, it can be observed that the accuracy values for Decision Tree, Logistic Regression, and Naïve Bayes reduced compared to the original dataset results, while Gradient Boosted Tree and Random Forest demonstrate improved accuracy. A similar trend is also observed in the other metrics including AUC values, where Gradient Boosted Tree and Random Forest exhibit enhanced AUC values, while other classifiers experience minor reductions. These fluctuations in performance can be attributed to the reduced dataset size resulting from random under sampling. While under sampling mitigates class imbalance, it also leads to a decrease in the overall amount of training data available for the models. Therefore, some classifiers, particularly those relying on intricate patterns, encounters limitations in their ability to capture complex relationships within the data, thereby resulting in marginal decreases in accuracy and AUC. Conversely, the improvement observed for Gradient Boosted Tree and Random Forest could stem from their inherent resilience to small dataset sizes and their capacity to harness the available data effectively. When comparing training and testing results, it also shows significant overfitting for these models.


\subsubsection{NearMiss}

Table \ref{tab:Tuned_Hyperparameters_NearMiss} shows the result of hyper parameter tuning for NearMiss sampled dataset. The Decision Tree model showcased improved predictive performance with \verb|class_weight| set to ‘balanced’, ‘criterion’ employing ‘gini’, \verb|max_depth| limited to 5, \verb|min_samples_leaf| set to 2, and \verb|min_samples_split| of 16. In parallel, the Gradient Boosted Tree model’s performance experienced an upswing with an optimal \verb|learning_rate| of 0.3161, \verb|max_depth| restricted to 2, \verb|min_samples_leaf| of 0.1817, \verb|min_samples_split| of 0.4387, \verb|n_estimators| reaching 800, and ‘subsample’ amounting to 0.6105. The Logistic Regression model showcased optimal performance with parameter ‘C’ set to 0.0084, \verb|class_weight| as ‘balanced’, \verb|max_iter| capped at 10336, ‘penalty’ employing ‘l1’, and the ‘liblinear’ ‘solver’. Naïve Bayes had optimal performance with ‘prior’ of [0.3,0.7] and  \verb|var_smoothing| of 3.079e-05. The Random Forest model demonstrated optimal performance with parameters ‘bootstrap’ as false, \verb|class_weight| embracing \verb|balanced_subsample|, \verb|max_depth| expanded to 150, \verb|min_samples_leaf| set to 7, \verb|min_samples_split| at 11, and \verb|n_estimators| reaching 350.

\begin{table*}[t]
\begin{tabular}{|p{4cm}p{13cm}|} % use small p for left align column
\textbf{Model}        & \textbf{Parameters}                                                                                                                                                                       \\
Decision Tree         & \{‘class\_weight’: ‘balanced’, ‘criterion’: ‘gini’, ‘max\_depth’: 5, ‘max\_features’: None, ‘min\_samples\_leaf’: 2, ‘min\_samples\_split’: 16\}                                          \\
Gradient Boosted Tree & \{‘learning\_rate’: 0.3161, ‘max\_depth’: 2, ‘max\_features’: None, ‘min\_samples\_leaf’: 0.18175331720247354, ‘min\_samples\_split’: 0.4387, ‘n\_estimators’: 800, ‘subsample’: 0.6105\} \\
Logistic Regression   & \{‘C’: 0.0084, ‘class\_weight’: ‘balanced’, ‘max\_iter’: 10336, ‘penalty’: ‘l1’, ‘solver’: ‘liblinear’\}                                                                                  \\
Naïve Bayes           & \{‘priors’: {[}0.3, 0.7{]}, ‘var\_smoothing’: 3.079e-05\}                                                                                                                                 \\
Random Forest         & \{‘bootstrap’: false, ‘class\_weight’: ‘balanced\_subsample’, ‘max\_depth’: 150, ‘max\_features’: ‘log2’, ‘min\_samples\_leaf’: 7, ‘min\_samples\_split’: 11, ‘n\_estimators’: 350\}     
\end{tabular}
\caption{\label{tab:Tuned_Hyperparameters_NearMiss} Tuned Hyperparameters for the machine learning models with NearMiss sampled dataset.}
\end{table*}

Table \ref{tab:performance_NearMiss} shows the performance of the models with NearMiss sampled dataset. The Decision Tree and Gradient Boosted Tree models exhibit comparable accuracy and AUC values for both the training and testing datasets, indicating good generalisation. It can also be noted that Decision Tree achieve similar score across both training and testing dataset indicating a good fitting model. Logistic Regression and Naive Bayes achieve lower accuracy and AUC scores, particularly in the testing dataset, implying some difficulty in adapting to unseen data. Notably, the Random Forest model demonstrates higher accuracy and AUC values on the training set; however, it experiences a decrease in performance on the testing set, indicating overfitting.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\begin{tabular}{cc
>{\columncolor[HTML]{FFFF00}}c cccc}
\multicolumn{2}{c}{\textbf{}}                                     & \textbf{Decision Tree} & \textbf{Gradient Boosted Tree} & \textbf{Logistic Regression} & \textbf{Naive Bayes} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.018                  & 2.255                          & 0.043                        & 0.005                & 4.018                  \\
                                    & \textbf{Accuracy}           & 0.709                  & 0.749                          & 0.641                        & 0.673                & 0.845                  \\
                                    & \textbf{Weighted F1-Score}  & 0.708                  & 0.749                          & 0.637                        & 0.663                & 0.845                  \\
                                    & \textbf{Weighted Precision} & 0.710                  & 0.751                          & 0.646                        & 0.694                & 0.845                  \\
                                    & \textbf{Weighted Recall}    & 0.709                  & 0.749                          & 0.641                        & 0.673                & 0.845                  \\
                                    & \textbf{AUC}                & 0.709                  & 0.749                          & 0.641                        & 0.673                & 0.845                  \\
\multirow{-7}{*}{\textbf{Training}} & \textbf{Error}              & 0.291                  & 0.251                          & 0.359                        & 0.327                & 0.155                  \\
                                    & \textbf{Time (s)}           & 0.001                  & 0.021                          & 0.002                        & 0.001                & 0.167                  \\
                                    & \textbf{Accuracy}           & 0.709                  & 0.634                          & 0.484                        & 0.572                & 0.553                  \\
                                    & \textbf{Weighted F1-Score}  & 0.744                  & 0.682                          & 0.547                        & 0.628                & 0.608                  \\
                                    & \textbf{Weighted Precision} & 0.824                  & 0.833                          & 0.740                        & 0.754                & 0.814                  \\
                                    & \textbf{Weighted Recall}    & 0.709                  & 0.634                          & 0.484                        & 0.572                & 0.553                  \\
                                    & \textbf{AUC}                & 0.702                  & 0.703                          & 0.522                        & 0.553                & 0.649                  \\
\multirow{-7}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.291                  & 0.366                          & 0.516                        & 0.428                & 0.447                 
\end{tabular}
\caption{\label{tab:performance_NearMiss} The performance of machine learning models on the NearMiss sampled dataset.}
\end{table*}


\subsubsection{ENN}
For the Decision Tree model, the adoption of \verb|class_weight| as ‘balanced’, ‘criterion’ using ‘gini’, \verb|max_depth| capped at 5, \verb|min_samples_leaf| set to 17, and \verb|min_samples_split| at 8 contributed to improved predictive accuracy. In the case of the Gradient Boosted Tree, an optimal \verb|learning_rate| of 0.1106, a \verb|max_depth| of 8, \verb|max_features| utilizing ‘sqrt’, \verb|min_samples_leaf| of 0.0354, \verb|min_samples_split| of 0.0578, \verb|n_estimators| reaching 450, and ‘subsample’ set to 0.8939 yielded notable performance gains. The Logistic Regression model achieved enhanced outcomes by refining ‘C’ to 4.451, adopting \verb|class_weight| as ‘balanced’, setting \verb|max_iter| at 10386, employing ‘l2’ ‘penalty’, and using the ‘liblinear’ ‘solver’. Naive Bayes demonstrated favorable results with ‘priors’ adjusted to [0.5, 0.5] and \verb|var_smoothing| set at 3.798e-07. Additionally, the Random Forest model exhibited improved performance with parameters such as ‘bootstrap’ set to true, \verb|class_weight| embracing \verb|balanced_subsample|, \verb|max_depth| reaching 99, \verb|max_features| utilizing ‘sqrt’, \verb|min_samples_leaf| set at 18, \verb|min_samples_split| at 20, and \verb|n_estimators| extending to 950.

\begin{table*}[t]
\begin{tabular}{|p{4cm}p{13cm}|} % use small p for left align column
\textbf{Model}        & \textbf{Hyperparameters}                                                                                                                                                            \\
Decision Tree         & \{‘class\_weight’: ‘balanced’, ‘criterion’: ‘gini’, ‘max\_depth’: 5, ‘max\_features’: None, ‘min\_samples\_leaf’: 17, ‘min\_samples\_split’: 8\}                                    \\
Gradient Boosted Tree & \{‘learning\_rate’: 0.1106, ‘max\_depth’: 8, ‘max\_features’: ‘sqrt’, ‘min\_samples\_leaf’: 0.0354, ‘min\_samples\_split’: 0.0578, ‘n\_estimators’: 450, ‘subsample’: 0.8939\}      \\
Logistic Regression   & \{‘C’: 4.451, ‘class\_weight’: ‘balanced’, ‘max\_iter’: 10386, ‘penalty’: ‘l2’, ‘solver’: ‘liblinear’\}                                                                             \\
Naive Bayes           & \{‘priors’: {[}0.5, 0.5{]}, ‘var\_smoothing’: 3.798e-07\}                                                                                                                           \\
Random Forest         & \{‘bootstrap’: true, ‘class\_weight’: ‘balanced\_subsample’, ‘max\_depth’: 99, ‘max\_features’: ‘sqrt’, ‘min\_samples\_leaf’: 18, ‘min\_samples\_split’: 20, ‘n\_estimators’: 950\}
\end{tabular}
\caption{\label{tab:Tuned_Hyperparameters_ENN} Tuned Hyperparameters for the machine learning models with ENN sampled dataset.}
\end{table*}

Table \ref{tab:performance_ENN} shows the performance of the machine learning models after tuning. From the table it can be observed that The Decision Tree model achieved an accuracy of 0.739 on the training data, indicating that it correctly classified approximately 73.9\% of the instances. The corresponding AUC value of 0.790 suggests that its ability to discriminate between positive and negative classes is reasonably good. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\begin{tabular}{cc
>{\columncolor[HTML]{00FF00}}c 
>{\columncolor[HTML]{FFFF00}}c ccc}
\multicolumn{2}{c}{\textbf{}}                                     & \textbf{Decision Tree} & \textbf{Gradient Boosted Tree} & \textbf{Logistic Regression} & \textbf{Naive Bayes} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.034                  & 4.633                          & 0.095                        & 0.004                & 12.486                 \\
                                    & \textbf{Accuracy}           & 0.739                  & 0.902                          & 0.632                        & 0.687                & 0.797                  \\
                                    & \textbf{Weighted F1-Score}  & 0.758                  & 0.899                          & 0.657                        & 0.705                & 0.810                  \\
                                    & \textbf{Weighted Precision} & 0.837                  & 0.900                          & 0.715                        & 0.741                & 0.861                  \\
                                    & \textbf{Weighted Recall}    & 0.739                  & 0.902                          & 0.632                        & 0.687                & 0.797                  \\
                                    & \textbf{AUC}                & 0.790                  & 0.840                          & 0.618                        & 0.658                & 0.833                  \\
\multirow{-7}{*}{\textbf{Training}} & \textbf{Error}              & 0.261                  & 0.098                          & 0.368                        & 0.313                & 0.203                  \\
                                    & \textbf{Time (s)}           & 0.001                  & 0.052                          & 0.002                        & 0.001                & 0.373                  \\
                                    & \textbf{Accuracy}           & 0.657                  & 0.787                          & 0.594                        & 0.637                & 0.683                  \\
                                    & \textbf{Weighted F1-Score}  & 0.701                  & 0.797                          & 0.647                        & 0.683                & 0.725                  \\
                                    & \textbf{Weighted Precision} & 0.859                  & 0.811                          & 0.772                        & 0.788                & 0.848                  \\
                                    & \textbf{Weighted Recall}    & 0.657                  & 0.787                          & 0.594                        & 0.637                & 0.683                  \\
                                    & \textbf{AUC}                & 0.750                  & 0.668                          & 0.588                        & 0.623                & 0.741                  \\
\multirow{-7}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.343                  & 0.213                          & 0.406                        & 0.363                & 0.317                 
\end{tabular}
\caption{\label{tab:performance_ENN} The performance of machine learning models on the ENN sampled dataset}
\end{table*}

However, on the testing dataset, its accuracy dropped to 0.657, and the AUC remained comparable at 0.750. In contrast, the Gradient Boosted Tree model demonstrated higher accuracy and AUC values on both training and testing datasets. With an accuracy of 0.902 on the training data and an AUC of 0.840, this model exhibited a strong ability to capture intricate patterns and relationships in the data. This pattern was also observed for the testing dataset, where the accuracy remained relatively high at 0.787, although the AUC decreased to 0.668. The Logistic Regression and Naive Bayes models showed lower accuracy and AUC values across both training and testing datasets. Logistic Regression achieved an accuracy of 0.632 on the training data and an AUC of 0.618, indicating its moderate performance in capturing the data's underlying trends. Naive Bayes had an accuracy of 0.687 and an AUC of 0.658 on the training data. These models faced a slight decrease in accuracy and AUC on the testing dataset. The Random Forest model showcased a balanced performance with accuracy values of 0.797 and 0.683 on the training and testing datasets, respectively. Its AUC of 0.833 on the training data and 0.741 on the testing data suggests a solid ability to classify instances accurately and discriminate between classes.

\subsubsection{RENN}
Table \ref{tab:Tuned_Hyperparameters_RENN} shows the tuned hyper parameters for RENN dataset. In the context of the Decision Tree model, selecting \verb|class_weight| as ‘balanced’, ‘criterion’ using ‘entropy’, \verb|max_depth| confined to 5, \verb|min_samples_leaf| set to 10, and \verb|min_samples_split| of 2 collectively contributed to enhanced predictive accuracy. Similarly, the Gradient Boosted Tree model exhibited optimal performance by adopting an optimal \verb|learning_rate| of 0.2916, a restricted \verb|max_depth| of 1, \verb|min_samples_leaf| at 0.1039, \verb|min_samples_split| of 0.3341, \verb|n_estimators| reaching 750, and ‘subsample’ of 0.9636. The Logistic Regression model’s performance was increased with  ‘C’ value of 5.503, \verb|class_weight| as ‘balanced’, a maximum of 10130 \verb|max_iter|, ‘penalty’ employing ‘l1’, and utilizing the ‘liblinear’ ‘solver’. Naive Bayes demonstrated optimal results with prior of [0.5,0.5] and \verb|var_smoothing| at 8.2921e-07. Similarly, the Random Forest model exhibited improved performance with parameters such as ‘bootstrap’ set to true, \verb|class_weight| embracing ‘balanced’, \verb|max_depth| reaching 128, \verb|max_features| utilizing ‘log2’, \verb|min_samples_leaf| set at 16, \verb|min_samples_split| at 9, and \verb|n_estimators| extending to 200.

\begin{table*}[t]
\begin{tabular}{|p{4cm}p{13cm}|} % use small p for left align column
\textbf{Model}        & \textbf{Hyperparameters}                                                                                                                                                     \\
Decision Tree         & \{‘class\_weight’: ‘balanced’, ‘criterion’: ‘entropy’, ‘max\_depth’: 5, ‘max\_features’: None, ‘min\_samples\_leaf’: 10, ‘min\_samples\_split’: 2\}                          \\
Gradient Boosted Tree & \{‘learning\_rate’: 0.2916, ‘max\_depth’: 1, ‘max\_features’: None, ‘min\_samples\_leaf’: 0.1039, ‘min\_samples\_split’: 0.3341, ‘n\_estimators’: 750, ‘subsample’: 0.9636\} \\
Logistic Regression   & \{‘C’: 5.503, ‘class\_weight’: ‘balanced’, ‘max\_iter’: 10130, ‘penalty’: ‘l1’, ‘solver’: ‘liblinear’\}                                                                      \\
Naive Bayes           & \{‘priors’: {[}0.5, 0.5{]}, ‘var\_smoothing’: 8.2921e-07\}                                                                                                                   \\
Random Forest         & \{‘bootstrap’: true, ‘class\_weight’: ‘balanced’, ‘max\_depth’: 128, ‘max\_features’: ‘log2’, ‘min\_samples\_leaf’: 16, ‘min\_samples\_split’: 9, ‘n\_estimators’: 200\}    
\end{tabular}
\caption{\label{tab:Tuned_Hyperparameters_RENN} Tuned Hyperparameters for the machine learning models with RENN sampled dataset.}
\end{table*}

Table \ref{tab:performance_RENN} the performance of machine learning models for the RENN sampled dataset. The Decision Tree model achieved an accuracy of 0.790 on the training data, with an AUC of 0.818. However, on the testing data, the accuracy dropped to 0.660, and the AUC decreased slightly to 0.755. The Gradient Boosted Tree model performed well with an accuracy of 0.815 and an AUC of 0.787 on the training data, translating to an accuracy of 0.738 and an AUC of 0.727 on the testing data. In contrast, the Logistic Regression model had lower accuracy scores, reaching 0.650 on the training data and 0.584 on the testing data, with AUC values of 0.638 and 0.586, respectively. Naive Bayes demonstrated accuracy of 0.714 on the training data and 0.636 on the testing data, accompanied by AUC values of 0.682 and 0.623. Finally, the Random Forest model achieved an accuracy of 0.825 and an AUC of 0.848 on the training data, which decreased to an accuracy of 0.662 and an AUC of 0.741 on the testing data.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\begin{tabular}{cc
>{\columncolor[HTML]{00FF00}}c 
>{\columncolor[HTML]{FFFF00}}c ccc}
\multicolumn{2}{l}{}                                              & \textbf{Decision Tree} & \textbf{Gradient Boosted Tree} & \textbf{Logistic Regression} & \textbf{Naive Bayes} & \textbf{Random Forest} \\
                                    & \textbf{Time (s)}           & 0.032                  & 4.957                          & 38.265                       & 0.004                & 1.924                  \\
                                    & \textbf{Accuracy}           & 0.790                  & 0.815                          & 0.650                        & 0.714                & 0.825                  \\
                                    & \textbf{Weighted F1-Score}  & 0.799                  & 0.816                          & 0.663                        & 0.720                & 0.831                  \\
                                    & \textbf{Weighted Precision} & 0.838                  & 0.818                          & 0.693                        & 0.729                & 0.861                  \\
                                    & \textbf{Weighted Recall}    & 0.790                  & 0.815                          & 0.650                        & 0.714                & 0.825                  \\
                                    & \textbf{AUC}                & 0.818                  & 0.787                          & 0.638                        & 0.682                & 0.848                  \\
\multirow{-7}{*}{\textbf{Training}} & \textbf{Error}              & 0.210                  & 0.185                          & 0.350                        & 0.286                & 0.175                  \\
                                    & \textbf{Time (s)}           & 0.001                  & 0.024                          & 0.002                        & 0.001                & 0.077                  \\
                                    & \textbf{Accuracy}           & 0.660                  & 0.738                          & 0.584                        & 0.636                & 0.662                  \\
                                    & \textbf{Weighted F1-Score}  & 0.704                  & 0.768                          & 0.639                        & 0.683                & 0.706                  \\
                                    & \textbf{Weighted Precision} & 0.861                  & 0.835                          & 0.772                        & 0.788                & 0.852                  \\
                                    & \textbf{Weighted Recall}    & 0.660                  & 0.738                          & 0.584                        & 0.636                & 0.662                  \\
                                    & \textbf{AUC}                & 0.755                  & 0.727                          & 0.586                        & 0.623                & 0.741                  \\
\multirow{-7}{*}{\textbf{Testing}}  & \textbf{Error}              & 0.340                  & 0.262                          & 0.416                        & 0.364                & 0.338                 
\end{tabular}
\caption{\label{tab:performance_RENN} The performance of machine learning models on the RENN sampled dataset.}
\end{table*}


%%%%% at page 12 of 19. Just up to SMOTE
